Mitigating Spurious Correlations in Weakly Supervised Semantic Segmentation via Cross-architecture Consistency Regularization

Scarcity of pixel-level labels is a significant challenge in practical scenarios. In specific domains like industrial smoke, acquiring such detailed annotations is particularly difficult and often requires expert knowledge. To alleviate this, weakly supervised semantic segmentation (WSSS) has emerged as a promising approach. However, due to the supervision gap and inherent bias in models trained with only image level labels, existing WSSS methods suffer from limitations such as incomplete foreground coverage, inaccurate object boundaries, and spurious correlations, especially in our domain, where emissions are always spatially coupled with chimneys. Previous solutions typically rely on additional priors or external knowledge to mitigate these issues, but they often lack scalability and fail to address the model's inherent bias toward co-occurring context. To address this, we propose a novel WSSS framework that directly targets the co-occurrence problem without relying on external supervision. Unlike prior methods that adopt a single network, we employ a teacher-student framework that combines CNNs and ViTs. We introduce a knowledge transfer loss that enforces cross-architecture consistency by aligning internal representations. Additionally, we incorporate post-processing techniques to address partial coverage and further improve pseudo mask quality.

==> content/Preliminaries.tex <==
\chapter{Preliminaries}
In this section,we briefly recall preliminaries associated with weakly supervised semantic segmentation with image-level annotation.


\section{Vision Transformer Basics}
Vision Transformer,~ known for its strong capability to model long-range contexts dependency, firstly splits an image into $h\times w$ non-overlapping patches to form the initial patch tokens,~where each patch is flattened and linearly projected to form $h\times w$ tokens.
Then the patch tokens are concatenated with an extra learnable class token and feed into the Transformer encoder to obtain the final patch and class tokens. 
As the key component, in each Transformer block, the multi-head self-attention is used to perform the global feature dependency.
Specifically, in the context of our downstream task,~ViT features explicitly contain the contours and object boundaries.
This information is directly accessible in the self-attention modules of the last block \cite{caron2021emerging}.


\section{Knowledge Distillation}
Knowledge distillation concept was first proposed in~\cite{hinton2015distilling}, where the student network learns from both the ground truth labels and the soft-labels provided by the teacher model.~Typically, the teacher model~(pretrained) is more powerful and knowledgeable than the student model.~Given a teacher model $T$, a student model $S$, we denote $f^T$ and $f^S$ as the outputs of teacher and student network, which can be the activation of the outputs or intermediate feature maps. ~The conventional knowledge distillation methods can be formulated as follows:
\begin{equation}\label{eq:contrastive}
\mathcal{L}_{\text{KD}} =KL(softmax(\frac{f^S}{Tempeturature}),softmax(\frac{f^T}{Tempeturature}))
\end{equation}

The knowledge distillation can be applied for multiple distillation objectives,~including knowledge compression, knowledge enhancement, knowledge adaptation, and knowledge expansion~\cite{hu2023teacher}.
The objective of knowledge enhancement is to train student networks with more generalized feature representations under the guidance of specialized teacher networks, which is the goal our framework intends to achieve.

\section{Classification Activation Map}
CAM~\cite{zhou2016learning} is computed from a classification model to visualize the most discriminative regions related to the specific classes.
WSSS mainly relies on CAM to get coarse spatial information.~The class activation map  is generated by replacing the fully-connected layer of the classifier with the global average pooling layer.
The vanilla class activation maps are generated from the last convolutional layer of CNNs.

Given the classifier, the CAM of a ground truth class $c$, which is denoted by$M_c$,is computed as

\begin{equation}\label{eq:contrastive}
M_c(x,y)=w^T_cf^{cam}(x,y)
\end{equation}

where $w_c$ is the classification weights associated to the class $c$ and $f^{cam}(x,y)$ indicates the feature vector located at (x,y) on the feature map(last layer) before the global average pooling.
CAM is achieved by weighting the contribution of
each channel of the feature map to a specific category of the classification score.~Technically, for each class, we use two components to compute CAM: the feature map block after the last layer and  the weight for that class.~In this paper, we adopt the class activation map  as the initial pseudo-label.


\section{Segment Anything Model}
Segment Anything Model (SAM)~\cite{kirillov2023segment} is a recently proposed powerful visual foundation model. Its outstanding quality in segmentation makes it a promising way to handle all kinds of computer vision tasks. ~SAM can be utilized in various ways--either as a backbone to extract semantic features or by leveraging its pretrained knowledge to enhance downstream tasks.
SAM  consists of three key components: an image encoder, a prompt encoder and a mask decoder.~When using SAM as a pretrained model for feature extraction, only the image encoder is required.~When applying SAM for post-processing, the prompt encoder and mask decoder are employed to refine pseudo masks.
% \begin{itemize}
%     \item Grad-CAM,a generalization of CAM
%     \item Score-CAM
%     \item Layer-CAM:fuse from different layers of CNN
%         % \begin{itemize}
%         % \item[o] Item 4.1
%         % \end{itemize}
%     \item Norm-Grad
%     \item TS-CAM:the first Transformers-based method.
% \end{itemize}


% \subsubsection{Multi-stage }
% Multi-stage is a mainstream approach but suffer from high training costs.
% The first stage is to generate initial CAMs via a classification network,then refining the seed to produce a pseudo-mask and finally training fully supervised semantic segmentation models with the generated pseudo-mask.
% \paragraph{Generating Initial CAM Stage}

% \paragraph{Refining Initial CAM Stage}
% Traditional methods generate pseudo masks from CAMs by applying a global threshold, which can’t fully utilize CAMs due to ignorance of confidence information.
% \paragraph{Training Segmentation Model Stage}
% There is an inconsistency between the quality of the pseudo-labels and the performance of the final segmentation model\cite{rong2023boundary}.



% CNN would cause partial activation issue.This is the first attempt for using visual transformer for weakly supervised image task\cite{gao2021tscamtokensemanticcoupled}.
% There is a standard vision transformer as the encoder to realize classification and a lightweight decoder to make segmentation predictions.


% \subsubsection{DeepLabV3}
% ASPP module can aggregates spatial regularly sampled pixels at different dilated rates.

% \cite{papandreou2015weaklysemisupervisedlearningdcnn}.


% Existing  approaches can be categorized into mainly two direction.CAM based and multiple instance learning based.

% Use DeepLabv3 as the endocer module and add a simple yet effective decoder module to obtain sharper segmentations
% \cite{chen2018encoderdecoderatrousseparableconvolution}.

% ;Most weakly supervised learning moethods with image-level class labels are based on a class activation map.

% Despite being trained on image-level labels,CNNs have the remarkable ability to localize objects.

% global average pooling 

% the discriminative areas highlighted by CAMs are in turn used as seeds that will be propagated to cover the entire object area.
% \cite{zhou2016learning}.



% \subsubsection{Pixel-level Affinity}
% 
% The trained AffinityNet is used to revise CAMs of training images.



==> content/acknowledgement.tex <==
\section*{Acknowledgement} % * title not in table of contents

First and foremost, I would like to express my deep gratitude to my supervisor,~Prof. Yen Chia Hsu, for his support,~insight and invaluable feedback throughout the course of this thesis.~His expertise and patience have been instrumental in shaping both the methodology and the final outcomes of this work.~Without him, this thesis would have not been the same.

\noindent
I am also grateful to my second reader, Prof. Nanne van Noord, for his willingness to be the second reader and for taking the time to review my thesis.

\noindent
Also, I would like to thank my friends for their encouragement,~sharing knowledge and offering thoughtful feedback.~Especially, I wish to thank Miss Dong for her understanding during this journey.

\noindent
Last but not least, many thanks to my family for their unconditional love.

% \noindent\emph{"Going deeper. And still deeper – The green mountains."}
